Multi-modal AsynDGAN: Learn From Distributed Medical Image Data without Sharing Private Information

As deep learning technologies advance, increasingly more data is necessary to generate general and robust models for various tasks. In the medical domain, however, large-scale and multi-parties data training and analyses are infeasible due to the privacy and data security concerns. In this paper, we propose an extendable and elastic learning framework to preserve privacy and security while enabling collaborative learning with efficient communication. The proposed framework is named distributed Asynchronized Discriminator Generative Adversarial Networks (AsynDGAN), which consists of a centralized generator and multiple distributed discriminators. The advantages of our proposed framework are five-fold: 1) the central generator could learn the real data distribution from multiple datasets implicitly without sharing the image data; 2) the framework is applicable for single-modality or multi-modality data; 3) the learned generator can be used to synthesize samples for down-stream learning tasks to achieve close-to-real performance as using actual samples collected from multiple data centers; 4) the synthetic samples can also be used to augment data or complete missing modalities for one single data center; 5) the learning process is more efficient and requires lower bandwidth than other distributed deep learning methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> asyndgan <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{lecun2015deep}
Y.~LeCun, Y.~Bengio, and G.~Hinton, ``Deep learning,'' \emph{nature}, vol. 521,
  no. 7553, pp. 436--444, 2015.

\bibitem{litjens2017survey}
G.~Litjens, T.~Kooi, B.~E. Bejnordi, A.~A.~A. Setio, F.~Ciompi, M.~Ghafoorian,
  J.~A. Van Der~Laak, B.~Van~Ginneken, and C.~I. S{\'a}nchez, ``A survey on
  deep learning in medical image analysis,'' \emph{Medical image analysis},
  vol.~42, pp. 60--88, 2017.

\bibitem{shen2017deep}
D.~Shen, G.~Wu, and H.-I. Suk, ``Deep learning in medical image analysis,''
  \emph{Annual review of biomedical engineering}, vol.~19, pp. 221--248, 2017.

\bibitem{domingos2012few}
P.~M. Domingos, ``A few useful things to know about machine learning.''
  \emph{Commun. acm}, vol.~55, no.~10, pp. 78--87, 2012.

\bibitem{annas2003hipaa}
G.~J. Annas \emph{et~al.}, ``Hipaa regulations-a new era of medical-record
  privacy?'' \emph{New England Journal of Medicine}, vol. 348, no.~15, pp.
  1486--1490, 2003.

\bibitem{gostin2009beyond}
L.~O. Gostin, L.~A. Levit, S.~J. Nass \emph{et~al.}, \emph{Beyond the HIPAA
  privacy rule: enhancing privacy, improving health through research}.\hskip
  1em plus 0.5em minus 0.4em\relax National Academies Press, 2009.

\bibitem{regulation2018general}
P.~Regulation, ``General data protection regulation,'' \emph{Intouch}, 2018.

\bibitem{bankert2006institutional}
E.~A. Bankert and R.~J. Amdur, \emph{Institutional review board: Management and
  function}.\hskip 1em plus 0.5em minus 0.4em\relax Jones \& Bartlett Learning,
  2006.

\bibitem{mirsky2019ct}
Y.~Mirsky, T.~Mahler, I.~Shelef, and Y.~Elovici, ``{CT-GAN}: Malicious
  tampering of 3d medical imagery using deep learning,'' \emph{arXiv preprint
  arXiv:1901.03597}, 2019.

\bibitem{seddon2013cloud}
J.~J. Seddon and W.~L. Currie, ``Cloud computing and trans-border health data:
  Unpacking us and eu healthcare regulation and compliance,'' \emph{Health
  policy and technology}, vol.~2, no.~4, pp. 229--241, 2013.

\bibitem{kerikmae2017challenges}
M.~S.~T. Kerikm{\"a}e, ``Challenges in the e-health regulatory policy,''
  \emph{HOW DEEP IS YOUR LAW? BREXIT. TECHNOLOGIES. MODERN CONFLICTS}, vol.
  367, 2017.

\bibitem{menze2014multimodal}
B.~H. Menze, A.~Jakab, S.~Bauer, J.~Kalpathy-Cramer, K.~Farahani, J.~Kirby,
  Y.~Burren, N.~Porz, J.~Slotboom, R.~Wiest \emph{et~al.}, ``The multimodal
  brain tumor image segmentation benchmark ({BRATS}),'' \emph{IEEE transactions
  on medical imaging}, vol.~34, no.~10, pp. 1993--2024, 2014.

\bibitem{guo2019deep}
Z.~Guo, X.~Li, H.~Huang, N.~Guo, and Q.~Li, ``Deep learning-based image
  segmentation on multimodal medical imaging,'' \emph{IEEE Transactions on
  Radiation and Plasma Medical Sciences}, vol.~3, no.~2, pp. 162--169, 2019.

\bibitem{ivsgum2015evaluation}
I.~I{\v{s}}gum, M.~J. Benders, B.~Avants, M.~J. Cardoso, S.~J. Counsell, E.~F.
  Gomez, L.~Gui, P.~S. H{\H{u}}ppi, K.~J. Kersbergen, A.~Makropoulos
  \emph{et~al.}, ``Evaluation of automatic neonatal brain segmentation
  algorithms: the {NeoBrainS12} challenge,'' \emph{Medical image analysis},
  vol.~20, no.~1, pp. 135--151, 2015.

\bibitem{wang2019benchmark}
L.~Wang, D.~Nie, G.~Li, {\'E}.~Puybareau, J.~Dolz, Q.~Zhang, F.~Wang, J.~Xia,
  Z.~Wu, J.-W. Chen \emph{et~al.}, ``Benchmark on automatic six-month-old
  infant brain segmentation algorithms: The iseg-2017 challenge,'' \emph{IEEE
  transactions on medical imaging}, vol.~38, no.~9, pp. 2219--2230, 2019.

\bibitem{gao2019multi}
Y.~Gao, C.~Liu, and L.~Zhao, ``Multi-resolution path {CNN} with deep
  supervision for intervertebral disc localization and segmentation,'' in
  \emph{International Conference on Medical Image Computing and
  Computer-Assisted Intervention}.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2019, pp. 309--317.

\bibitem{zhou2019review}
T.~Zhou, S.~Ruan, and S.~Canu, ``A review: Deep learning for medical image
  segmentation using multi-modality fusion,'' \emph{Array}, p. 100004, 2019.

\bibitem{brown2018using}
A.~D. Brown and T.~R. Marotta, ``Using machine learning for sequence-level
  automated {MRI} protocol selection in neuroradiology,'' \emph{Journal of the
  American Medical Informatics Association}, vol.~25, no.~5, pp. 568--571,
  2018.

\bibitem{ellingson2015consensus}
B.~M. Ellingson, M.~Bendszus, J.~Boxerman, D.~Barboriak, B.~J. Erickson,
  M.~Smits, S.~J. Nelson, E.~Gerstner, B.~Alexander, G.~Goldmacher
  \emph{et~al.}, ``Consensus recommendations for a standardized brain tumor
  imaging protocol in clinical trials,'' \emph{Neuro-oncology}, vol.~17, no.~9,
  pp. 1188--1198, 2015.

\bibitem{aryanto2015free}
K.~Aryanto, M.~Oudkerk, and P.~van Ooijen, ``Free dicom de-identification tools
  in clinical research: functioning and safety of patient privacy,''
  \emph{European radiology}, vol.~25, no.~12, pp. 3685--3695, 2015.

\bibitem{cai2018deep}
L.~Cai, Z.~Wang, H.~Gao, D.~Shen, and S.~Ji, ``Deep adversarial learning for
  multi-modality missing data completion,'' in \emph{Proceedings of the 24th
  ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  2018, pp. 1158--1166.

\bibitem{chang2020synthetic}
Q.~Chang, H.~Qu, Y.~Zhang, M.~Sabuncu, C.~Chen, T.~Zhang, and D.~N. Metaxas,
  ``Synthetic learning: Learn from distributed asynchronized discriminator
  {GAN} without sharing medical image data,'' in \emph{Proceedings of the
  IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 2020, pp.
  13\,856--13\,866.

\bibitem{konevcny2016federated}
J.~Kone{\v{c}}n{\`y}, H.~B. McMahan, F.~X. Yu, P.~Richt{\'a}rik, A.~T. Suresh,
  and D.~Bacon, ``Federated learning: Strategies for improving communication
  efficiency,'' \emph{arXiv preprint arXiv:1610.05492}, 2016.

\bibitem{hard2018federated}
A.~Hard, K.~Rao, R.~Mathews, S.~Ramaswamy, F.~Beaufays, S.~Augenstein,
  H.~Eichner, C.~Kiddon, and D.~Ramage, ``Federated learning for mobile
  keyboard prediction,'' \emph{arXiv preprint arXiv:1811.03604}, 2018.

\bibitem{brisimi2018federated}
T.~S. Brisimi, R.~Chen, T.~Mela, A.~Olshevsky, I.~C. Paschalidis, and W.~Shi,
  ``Federated learning of predictive models from federated electronic health
  records,'' \emph{International journal of medical informatics}, vol. 112, pp.
  59--67, 2018.

\bibitem{huang2018loadaboost}
L.~Huang, Y.~Yin, Z.~Fu, S.~Zhang, H.~Deng, and D.~Liu, ``Loadaboost:
  Loss-based adaboost federated machine learning on medical data,'' \emph{arXiv
  preprint arXiv:1811.12629}, 2018.

\bibitem{wagner2018technical}
I.~Wagner and D.~Eckhoff, ``Technical privacy metrics: a systematic survey,''
  \emph{ACM Computing Surveys (CSUR)}, vol.~51, no.~3, pp. 1--38, 2018.

\bibitem{dwork2014algorithmic}
C.~Dwork, A.~Roth \emph{et~al.}, ``The algorithmic foundations of differential
  privacy.'' \emph{Foundations and Trends in Theoretical Computer Science},
  vol.~9, no. 3-4, pp. 211--407, 2014.

\bibitem{abadi2016deep}
M.~Abadi, A.~Chu, I.~Goodfellow, H.~B. McMahan, I.~Mironov, K.~Talwar, and
  L.~Zhang, ``Deep learning with differential privacy,'' in \emph{Proceedings
  of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  2016, pp. 308--318.

\bibitem{gentry2009fully}
C.~Gentry and D.~Boneh, \emph{A fully homomorphic encryption scheme}.\hskip 1em
  plus 0.5em minus 0.4em\relax Stanford university Stanford, 2009, vol.~20,
  no.~9.

\bibitem{gentry2009fully2}
C.~Gentry, ``Fully homomorphic encryption using ideal lattices,'' in
  \emph{Proceedings of the forty-first annual ACM symposium on Theory of
  computing}, 2009, pp. 169--178.

\bibitem{orekondy2018gradient}
T.~Orekondy, S.~J. Oh, Y.~Zhang, B.~Schiele, and M.~Fritz, ``Gradient-leaks:
  Understanding and controlling deanonymization in federated learning,''
  \emph{arXiv preprint arXiv:1805.05838}, 2018.

\bibitem{melis2019exploiting}
L.~Melis, C.~Song, E.~De~Cristofaro, and V.~Shmatikov, ``Exploiting unintended
  feature leakage in collaborative learning,'' in \emph{2019 IEEE Symposium on
  Security and Privacy (SP)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2019, pp. 691--706.

\bibitem{mcmahan2016communication}
H.~B. McMahan, E.~Moore, D.~Ramage, S.~Hampson \emph{et~al.},
  ``Communication-efficient learning of deep networks from decentralized
  data,'' \emph{arXiv preprint arXiv:1602.05629}, 2016.

\bibitem{agarwal2018cpsgd}
N.~Agarwal, A.~T. Suresh, F.~X.~X. Yu, S.~Kumar, and B.~McMahan, ``cpsgd:
  Communication-efficient and differentially-private distributed sgd,'' in
  \emph{Advances in Neural Information Processing Systems}, 2018, pp.
  7564--7575.

\bibitem{jayaraman2018distributed}
B.~Jayaraman, L.~Wang, D.~Evans, and Q.~Gu, ``Distributed learning without
  distress: Privacy-preserving empirical risk minimization,'' in \emph{Advances
  in Neural Information Processing Systems}, 2018, pp. 6343--6354.

\bibitem{he2016resnet}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image
  recognition,'' in \emph{Proceedings of the IEEE conference on computer vision
  and pattern recognition}, 2016, pp. 770--778.

\bibitem{vepakomma2018split}
P.~Vepakomma, O.~Gupta, T.~Swedish, and R.~Raskar, ``Split learning for health:
  Distributed deep learning without sharing raw patient data,'' \emph{arXiv
  preprint arXiv:1812.00564}, 2018.

\bibitem{goodfellow2014generative}
I.~Goodfellow, J.~Pouget-Abadie, M.~Mirza, B.~Xu, D.~Warde-Farley, S.~Ozair,
  A.~Courville, and Y.~Bengio, ``Generative adversarial nets,'' in
  \emph{Advances in neural information processing systems}, 2014, pp.
  2672--2680.

\bibitem{hardy2019md}
C.~Hardy, E.~Le~Merrer, and B.~Sericola, ``{MD-GAN}: Multi-discriminator
  generative adversarial networks for distributed datasets,'' in \emph{2019
  IEEE International Parallel and Distributed Processing Symposium
  (IPDPS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2019, pp. 866--877.

\bibitem{li2014deep}
R.~Li, W.~Zhang, H.-I. Suk, L.~Wang, J.~Li, D.~Shen, and S.~Ji, ``Deep learning
  based imaging data completion for improved brain disease diagnosis,'' in
  \emph{International Conference on Medical Image Computing and
  Computer-Assisted Intervention}.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2014, pp. 305--312.

\bibitem{ioffe2015batch}
S.~Ioffe and C.~Szegedy, ``Batch normalization: Accelerating deep network
  training by reducing internal covariate shift,'' \emph{arXiv preprint
  arXiv:1502.03167}, 2015.

\bibitem{pix2pix2017}
P.~Isola, J.-Y. Zhu, T.~Zhou, and A.~A. Efros, ``Image-to-image translation
  with conditional adversarial networks,'' \emph{CVPR}, 2017.

\bibitem{li2016precomputed}
C.~Li and M.~Wand, ``Precomputed real-time texture synthesis with markovian
  generative adversarial networks,'' in \emph{European Conference on Computer
  Vision}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2016, pp. 702--716.

\bibitem{isola2017image}
P.~Isola, J.-Y. Zhu, T.~Zhou, and A.~A. Efros, ``Image-to-image translation
  with conditional adversarial networks,'' in \emph{Proceedings of the IEEE
  conference on computer vision and pattern recognition}, 2017, pp. 1125--1134.

\bibitem{mirza2014conditiongan}
M.~Mirza and S.~Osindero, ``Conditional generative adversarial nets,'' 2014.

\bibitem{mathieu2015deep}
M.~Mathieu, C.~Couprie, and Y.~LeCun, ``Deep multi-scale video prediction
  beyond mean square error,'' \emph{arXiv preprint arXiv:1511.05440}, 2015.

\bibitem{Johnson2016Perceptual}
J.~Johnson, A.~Alahi, and L.~Fei-Fei, ``Perceptual losses for real-time style
  transfer and super-resolution,'' in \emph{European Conference on Computer
  Vision}, 2016.

\bibitem{Zhang_2018_CVPR}
Z.~Zhang, L.~Yang, and Y.~Zheng, ``Translating and segmenting multimodal
  medical volumes with cycle- and shape-consistency generative adversarial
  network,'' in \emph{Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition (CVPR)}, June 2018.

\bibitem{bakas2017advancing}
S.~Bakas, H.~Akbari, A.~Sotiras, M.~Bilello, M.~Rozycki, J.~S. Kirby, J.~B.
  Freymann, K.~Farahani, and C.~Davatzikos, ``Advancing the cancer genome atlas
  glioma {MRI} collections with expert segmentation labels and radiomic
  features,'' \emph{Scientific data}, vol.~4, p. 170117, 2017.

\bibitem{bakas2018identifying}
S.~Bakas, M.~Reyes, A.~Jakab, S.~Bauer, M.~Rempfler, A.~Crimi, R.~T. Shinohara,
  C.~Berger, S.~M. Ha, M.~Rozycki \emph{et~al.}, ``Identifying the best machine
  learning algorithms for brain tumor segmentation, progression assessment, and
  overall survival prediction in the brats challenge,'' \emph{arXiv preprint
  arXiv:1811.02629}, 2018.

\bibitem{he2016deep}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image
  recognition,'' in \emph{Proceedings of the IEEE conference on computer vision
  and pattern recognition}, 2016, pp. 770--778.

\bibitem{kingma2014adam}
D.~P. Kingma and J.~Ba, ``Adam: A method for stochastic optimization,''
  \emph{arXiv preprint arXiv:1412.6980}, 2014.

\bibitem{antoniou2017data}
A.~Antoniou, A.~Storkey, and H.~Edwards, ``Data augmentation generative
  adversarial networks,'' \emph{arXiv preprint arXiv:1711.04340}, 2017.

\bibitem{arjovsky2017wasserstein}
M.~Arjovsky, S.~Chintala, and L.~Bottou, ``Wasserstein gan,'' \emph{arXiv
  preprint arXiv:1701.07875}, 2017.

\bibitem{mao2017least}
X.~Mao, Q.~Li, H.~Xie, R.~Y. Lau, Z.~Wang, and S.~Paul~Smolley, ``Least squares
  generative adversarial networks,'' in \emph{Proceedings of the IEEE
  International Conference on Computer Vision}, 2017, pp. 2794--2802.

\end{thebibliography}

